An Overview on the Generation and Detection of Synthetic and Manipulated Satellite Images

Due to the reduction of technological costs and the increase of satellites launches, satellite images are becoming more popular and easier to obtain. Besides serving benevolent purposes, satellite data can also be used for malicious reasons such as misinformation. As a matter of fact, satellite images can be easily manipulated relying on general image editing tools. Moreover, with the surge of Deep Neural Networks (DNNs) that can generate realistic synthetic imagery belonging to various domains, additional threats related to the diffusion of synthetically generated satellite images are emerging. In this paper, we review the State of the Art (SOTA) on the generation and manipulation of satellite images. In particular, we focus on both the generation of synthetic satellite imagery from scratch, and the semantic manipulation of satellite images by means of image-transfer technologies, including the transformation of images obtained from one type of sensor to another one. We also describe forensic detection techniques that have been researched so far to classify and detect synthetic image forgeries. While we focus mostly on forensic techniques explicitly tailored to the detection of AI-generated synthetic contents, we also review some methods designed for general splicing detection, which can in principle also be used to spot AI manipulate images

==> notation_helper.tex <==
\subsection{TEMP: notation helper}
Here are some ideas / suggestions to discuss together :)

\vspace{.5em}\noindent\textbf{General rules}
\begin{itemize}
    \item $x$ scalar variable (e.g., the class of an image)
    \item $X$ scalar constant (e.g., the number of classes)
    \item $\mathbf{x}$ vector (e.g., feature vector extracted by a network)
    \item $\mathbf{X}$ matrix / tensor (e.g., an image)
    \item $\emph{X}(\cdot)$ function / operator (e.g., a network forward pass)
    \item $\mathcal{X}$ sets (e.g., a dataset)
\end{itemize}

\vspace{.5em}\noindent\textbf{Input-output}
\begin{itemize}
    \item $\Xrgb$ input RGB image
        \begin{itemize}
            \item $\Xrgb[i, j]$ pixel in position $[i, j]$ (maybe not necessary)
        \end{itemize}
    \item $\Xsar$ input amplitude \gls{sar} image
    \item $\Xpan$ input panchromatic image
    \item $\P$ input image patch
        \begin{itemize}
            \item $\P^i$ $i$-th patch in an image $\X$ (maybe not necessary)
        \end{itemize}
    \item $\M$ ground truth binary mask
        \begin{itemize}
            \item $\M_\text{gt}$?
        \end{itemize}
    \item $\Msoft$ output forgery heatmap
        \begin{itemize}
            \item $\M_\text{float}$? $\M_\text{soft}$?
            \item We suggest $\Msoft$ as some methods have multiple outputs (e.g., $\Msoft_\text{KNN}$ and $\Msoft_\text{GMM}$)
        \end{itemize}
    \item $\Mbin$ output forgery binary mask
        \begin{itemize}
            \item $\M_\text{bool}$? $\M_\text{bin}$?
        \end{itemize}
    \item $\y$ ground truth label / class
        \begin{itemize}
            \item $c$ as class? $l$ as label? with or without $\Box_\text{gt}$?
        \end{itemize}
    \item $\ysoft$ tampering detection soft score
        \begin{itemize}
            \item $c$ as class? $l$ as label? $\Box_\text{soft}$ vs $\Box_\text{float}$ vs $\tilde{\Box}$?
        \end{itemize}
    \item $\ybin$ tampering detection binary label
        \begin{itemize}
            \item  $c$ as class? $l$ as label? $\Box_\text{bin}$ vs $\Box_\text{bool}$ vs $\hat{\Box}$?
        \end{itemize}
\end{itemize}

\vspace{.5em}\noindent\textbf{Methods}
\begin{itemize}
    \item $\emph{C}(\cdot)$ \gls{cnn} operator
        \begin{itemize}
            \item $\emph{A}$ $\Phi_\text{AE}()$ Autoencoder
            \item $\emph{A}_\text{e}$ $\Phi_\text{Enc}()$ Autoencoder encoder
            \item $\emph{A}_\text{d}$ Autoencoder decoder
            \item $\emph{G}$ \gls{gan} generator
            \item $\emph{D}$ \gls{gan} discriminator
        \end{itemize}
    \item $\emph{L}$ loss function
        \begin{itemize}
            \item $\emph{L}_{\ell1}$ $\ell1$ loss
            \item $\emph{L}_{\ell2}$ $\ell2$ loss
            \item $\emph{L}_\text{BCE}$ \gls{bce} loss
            \LA{here is it possible to superscript also with the loss representation? for example $\emph{L}_\text{BCE}^{adv}$ to represent adversarial loss?}
        \end{itemize}
    \item $\emph{c}(\cdot)$ generic machine-learning technique (e.g., classifier, clustering, etc.)
        \begin{itemize}
            \item $\emph{c}_\text{SVM}$ \gls{svm}
            \item $\emph{c}_\text{RF}$ \gls{rf}
            \item $\emph{c}_\text{KM}$ \gls{km}
            \item $\emph{c}_\text{GMM}$ \gls{gmm}
        \end{itemize}
\end{itemize}

%%%%adding annotation temporary in the same place
In addition to the annotations added in section IV-A, we need the ones below
\begin{itemize}
 \item $\hat{X}$ output generated image \textcolor{blue}{Suggestion: $\hat{\mathbf{X}}$}
 \item $R_{SAR,RGB,specific band}$ \textcolor{blue}{suggestion: $\Xrgb$,.. $\mathbf{X}_{13}$ : reference image}
 \item \textcolor{blue}{${f}()$  (feature extractor/encoder)}
 \item \textcolor{blue}{$\mathbf{f}$ o $\mathbf{x}$??? (feature vector extracted by the network)}
  \item \textcolor{blue}{${g}()$  (classification part of the network/decoder)}
 \item \textcolor{blue}{$\Phi()$ network output function}
 \item $s_{idx}$: style or domain the index represents the enumerated domain
\end{itemize}
%
